Investigating Vulnerabilities of GPS Trip Data to Trajectory-User Linking Attacks

Open human mobility data is considered an essential basis for the profound research and analysis required for the transition to sustainable mobility and sustainable urban planning. Cycling data has especially been the focus of data collection endeavors in recent years. Although privacy risks regarding location data are widely known, practitioners often refrain from advanced privacy mechanisms to prevent utility losses. Removing user identifiers from trips is thereby deemed a major privacy gain, as it supposedly prevents linking single trips to obtain entire movement patterns. In this paper, we propose a novel attack to reconstruct user identifiers in GPS trip datasets consisting of single trips, unlike previous ones that are dedicated to evaluating trajectory-user linking in the context of check-in data. We evaluate the remaining privacy risk for users in such datasets and our empirical findings from two real-world datasets show that the risk of re-identification is significant even when personal identifiers have been removed, and that truncation as a simple additional privacy mechanism may not be effective in protecting user privacy. Further investigations indicate that users who frequently visit locations that are only visited by a small number of others, tend to be more vulnerable to re-identification.

==> appendices/baselinelosscurves.tex <==
%TC:ignore
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{./img/e2dtc_freemove_curves.png}
    \caption{Loss curves and ARI for the E2DTC deep clustering framework and the \textit{freemove} dataset. Plots show loss curves during (A) trajectory representation learning and (B) cluster refinement step. The stagnating clustering performance indicates that the framework fails to capture the underlying user profiles from clustering spatio-temporal similar trajectories.}
    \label{Figure:e2dtc_freemove_curves}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{./img/e2dtc_geolife_curves.png}
    \caption{Loss curves and ARI for the E2DTC deep clustering framework and the \textit{GeoLife} dataset. Plots show loss curves during (A) trajectory representation learning and (B) cluster refinement step. The stagnating clustering performance indicates that the framework fails to capture the underlying user profiles from clustering spatio-temporal similar trajectories.}
    \label{Figure:e2dtc_geolife_curves}
\end{figure}
%TC:endignore




==> appendices/dataset.tex <==
%TC:ignore
\begin{figure}[H]
    \centering
    \includegraphics[width=10cm]{./img/box_berlin.png}
    \caption{Bounding box of tesselation used for Berlin and the freemove dataset. Trajectories starting or ending outside of this box are discarded.}
    \label{Figure:boxberlin}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=10cm]{./img/box_peking.png}
    \caption{Bounding box of tesselation used for Beijing and the GeoLife dataset. Trajectories starting or ending outside of this box are discarded.}
    \label{Figure:boxpeking}
\end{figure}




%TC:endignore

==> appendices/extendedresults.tex <==
%TC:ignore
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{./img/usercharacteristics_nrp_10.png}
    \caption{Mean F-scores given random points $L_{p=10}$ across mobility characteristics for users in (A) freemove and (B) GeoLife.}
    \label{Figure:usercharacteristics_nrp_10}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{./img/obfuscated.png}
    \caption{Performance across data types and grid cell sizes for various numbers of random spatio-temporal points assumed as knowledge of an attacker. (A) freemove and (B) GeoLife.}
    \label{Figure:obfuscated}
\end{figure}
%TC:endignore

==> appendices/methoddetails.tex <==
%TC:ignore
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{./img/dissolvingexample.png}
    \caption{Example illustration of adjacent HL tiles that would be dissolved into one combined polygon during the HL assignment step.}
    \label{Figure:dissolvingexample}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{./img/lcss.png}
    \caption{Example illustration of LCSS metric for a pair of trajectories. (A) being the original trips and (B) with the upper trajectory reverted. The LCSS value in (A) is 0.5 since 50\% of the points of the shorter trajectory are within a distance threshold $LCSS_{eps}$ from their counterpart in the longer trajectory. Analogously, in (B) the LCSS results in 0.25 because when comparing the points in reverted order -- the direction of travel for one of the trajectories goes in the opposite direction, only 25\% of the points are within $LCSS_{eps}$. Note here that for easier readability the red lines indicating points that are further apart than the specified threshold, are only plotted exemplary for two of the above point pairs.}
    \label{Figure:lcss}
\end{figure}

\subsubsection{Motivation for iterative TF-IDF refinement over standard clustering}\label{appendix:motivation_tfidf}

It is important to point out that I am not applying standard clustering techniques to the TF-IDF weighted location visit patterns to further refine our user ID mapping since the objective is not to find overall similar sets of trajectories but rather the highly relevant link that contains -- from an information-theoretic view -- high "amounts of information" \citep{aizawaInformationtheoreticPerspectiveTf2003}. In other words, this approach aims to link two otherwise disjoint sets of trajectories that reflect two behavior patterns of the same person. For example, instead of matching geospatially similar trips, such as all the commuters traveling to a business district starting in the same part of town, I identify if there is a trip connecting the HLs of an individual in our data and their hypothetical partner in case this person frequently stays over at their partner's apartment.

\begin{figure}[H]
    \centering
    \includegraphics[width=6cm]{./img/simra_trip.png}
    \caption{Screenshot of the SimRa app where users have the choice to truncate their trajectories by a variable margin set with a slider control around starting and end points.}
    \label{Figure:simratrip}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=6cm]{./img/simra_settings.png}
    \caption{Screenshot of the SimRa app's preferences showing the setting for truncating an initial segment of flexible length up to 50m for every trajectory by default.}
    \label{Figure:simrasettings}
\end{figure}

%TC:endignore

